Neuro CROSS exchange: Learning to CROSS exchange to solve realistic vehicle routing problems

CROSS exchange (CE), a meta-heuristic that solves various vehicle routing problems (VRPs), improves the solutions of VRPs by swapping the sub-tours of the vehicles. Inspired by CE, we propose Neuro CE (NCE), a fundamental operator of learned meta-heuristic, to solve various VRPs while overcoming the limitations of CE (i.e., the expensive $\mathcal{O}(n^4)$ search cost). NCE employs a graph neural network to predict the cost-decrements (i.e., results of CE searches) and utilizes the predicted cost-decrements as guidance for search to decrease the search cost to $\mathcal{O}(n^2)$. As the learning objective of NCE is to predict the cost-decrement, the training can be simply done in a supervised fashion, whose training samples can be prepared effortlessly. Despite the simplicity of NCE, numerical results show that the NCE trained with flexible multi-depot VRP (FMDVRP) outperforms the meta-heuristic baselines. More importantly, it significantly outperforms the neural baselines when solving distinctive special cases of FMDVRP (e.g., MDVRP, mTSP, CVRP) without additional training.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
  \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{} We will publicize the code after the decision.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{} We follow the convention of our targeting research community which reports the mean values.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> sections/03-2-NCE-cost-pred.tex <==
The proposed NCE operation is able to save computational budgets by predicting $y^*(\cdot)$ of Equation \ref{eqn:NCE-opt-dec-cost}. In this subsection, we explain how the cost-decrement prediction model $f_\theta(a_1,a_2;\tau_1,\tau_2)$ predicts $y^*(\cdot)$ from $a_1,a_2,\tau_1$, and $\tau_2$. The overall procedure is illustrated in \cref{fig:cost-decr-pred}.

\paragraph{Graph representation of $(\tau_1, \tau_2)$}
We represent the pair of tours $(\tau_1, \tau_2)$ as a directed complete graph $\gG=(\sN, \mathbb{E})$, where $\sN=\tau_1 \cup \tau_2$ (i.e., the $i^{\text{th}}$ node $n_i$ of $\gG$ is either the customer or depot of the tours and $e_{ij}$ is the edge from $v_i$ to $v_j$). However, $\gG$ cannot capture the ordinal/intra-tour information of within/among the tour(s) as it is. We encode such crucial information of $(\tau_1, \tau_2)$ into $\gG$, by defining the node feature $x_i$ and edge feature $x_{ij}$ as follows:

\begin{itemize}[leftmargin=0.5cm]
\vspace{-0.25cm}
    \item  $x_i \triangleq [\textbf{coord}(n_i), \mathbbm{1}_{\textbf{depot}}(n_i)]$, where $\textbf{coord}(n_i)$ is 2D Euclidean coordinate of $v_i$, and $\mathbbm{1}_{\textbf{depot}}(n_i)$ is the indicator whether $n_i$ is depot.
    \item $x_{ij} \triangleq [\textbf{dist}(n_i, n_j), \textbf{type}(n_i, n_j)]$, where $\textbf{dist}(n_i, n_j)$ is the 2D Euclidean distance between $n_i$ and $n_j$, and $\textbf{type}(n_i, n_j)$ gives the \textit{type} of $e_{ij}$. We design $\textbf{type}(n_i, n_j)$ so that it returns the one-hot vector representing the forward/backward relationship of nodes within the tour, and inter tour relationships. Refer to Appendix \textcolor{red}{!!} for the further details of $\textbf{type}(n_i, n_j)$.
\end{itemize}
\vspace{-0.25cm}
The use of $\textbf{type}(n_i, n_j)$ allows the following graph embedding procedure considers the order of sequences (i.e., the order of cities in the tours) and, additionally, the inter-tour information. The type information plays the similar role of the positional encoding of the transformers \cite{vaswani2017attention}.

\begin{figure}[t]
    \centering
    \includegraphics[width={\linewidth}]{figs/fig-gnn-cost-pred-cropped.pdf}
    \caption{Cost-decrement prediction procedure}
    \label{fig:cost-decr-pred}
\end{figure}

\paragraph{Graph embedding with attentive GNN} We employ an attentive variant of graph-network (GN) block \cite{battaglia2018relational} to embed $\gG$. The attentive embedding layer is defined as follows:
\begin{align}
\label{eq:gnn-layer}
h'_{ij} &= \phi_e(h_i,h_j,h_{ij},x_{ij}) \\
z_{ij} &= \phi_w(h_i,h_j,h_{ij},x_{ij}) \\ 
w_{ij} &= \softmax(\{z_{ij}\}_{j \in \mathcal{N}(i)}) \\    
h'_{i} &= \phi_n(h_i, \sum_{j \in \mathcal{N}(i)} w_{ij} h'_{ij})
\end{align}
where $h_i$ and $h_{ij}$ are node and edge embedding, respectively, $\phi_e$, $\phi_w$, and $\phi_n$ are Multilayer Perceptron (MLP)-parameterized edge, attention and node operators, respectively, and $\mathcal{N}(i)$ is the in-warding neighbors of $n_i$. We utilize $H$ embedding layers to compute the final node and $\{h^{(H)}_i |\, n_i\in \sV\}$ edge embeddings $\{h^{(H)}_{ij} | \, e_{ij}\in \mathbb{E}\}$.

\paragraph{Cost decrement prediction} Based on the computed embedding, the cost prediction module $\phi_c$ predicts $y^*(a_1,a_2;\tau_1,\tau_2)$. We interpret the selection of edge between $(a_1, a_2)$ -- the first search stage of the NCE operation -- as (1) the additions of the links between the node $a_1/a_2$ and $a_2+1/a_1+1$\footnote{We overload the notation $a_1+1, a_2+1$ so that they denote the next nodes of $a_1, a_2$ in $\tau_1, \tau_2$, respectively.}, and (2) the removals of the links between $a_1/a_2$ and $a_1+1/a_2+1$ to the tours, as shown in \cref{fig:cost-decr-pred} (Right). With such interpretation, the cost prediction is done as follows:
\begin{align}
\label{eq:cost-pred-layer}
\hat y^*(a_1,a_2;\tau_1,\tau_2)=\phi_c(
\underbrace{h^{(H)}_{a_1}, 
            h^{(H)}_{a_1+1}, 
            h^{(H)}_{a_2}, 
            h^{(H)}_{a_2+1}}_{\tikz\draw[NavyBlue, fill=NavyBlue] (0,0) circle (.5ex); /
                              \tikz\draw[Orange, fill=Orange] (0,0) circle (.5ex);
                              \textbf{ : node embedding}},
\underbrace{h^{(H)}_{a_1,a_2+1}, h^{(H)}_{a_2,a_1+1}}_
      {\tikz\draw[ForestGreen, thick] (0,1.0)--(0.3,1.0); 
       \textbf{ : link addition}},
\underbrace{h^{(H)}_{a_1,a_1+1}, h^{(H)}_{a_2,a_2+1}}_
      {\tikz\draw[ForestGreen, thick, densely dotted] (0,1.0)--(0.3,1.0);
      \textbf{ : link removal}}
)
\end{align}
where $h^{(H)}_x$ and $h^{(H)}_{x,y}$ denotes the embedding of node $x$ and edge from $x$ to $y$, respectively.

\paragraph{Prediction results} The quality of NCE operator (i.e., whether NCE operator finds the improving pairs) is highly depending on the accuracy of $f_\theta$. When $K \geq {10}$, we experimentally confirmed that the NCE operator finds the argmax pair of $(a_1,a_2,b_1,b_2)$ with a high probability. We provide the experimental details and results about the predictions of $f_\theta$ in \cref{}



==> tables/model_hparams.tex <==
\begin{table}
	\caption{Hyperparameters for Graph Attention Network}
	\label{params}
	\centering
	\small
	\begin{tabular}{cccc}
		\toprule
		Parameters (for Graph network) & Value & Parameters (for Supervise learning) & Value \\\midrule
		MLP units & $(64, 64)$& Optimizer & AdamW \\
		Neuron initialization & Xavier &betas ($\beta_1$, $\beta_2$) & $(0.9, 0.999)$ \\
		Activation fn. & Mish & Learning rate ($\eta_{policy}$) & $5 \times 10^{-4}$\\
		GNN update epoch ($N^{hop}$)  & 3 & Loss & Huberloss \\



		\bottomrule
	\end{tabular}
\end{table}	
